ASHiTA: Automatic Scene-grounded HIerarchical Task Analysis

While recent work in scene reconstruction and understanding has made strides in grounding natural language to physical 3D environments, it is still challenging to ground abstract, high-level instructions to a 3D scene. High-level instructions might not explicitly invoke semantic elements in the scene, and even the process of breaking a high-level task into a set of more concrete subtasks, a process called hierarchical task analysis, is environment-dependent. In this work, we propose ASHiTA, the first framework that generates a task hierarchy grounded to a 3D scene graph by breaking down high-level tasks into grounded subtasks. ASHiTA alternates LLM-assisted hierarchical task analysis, to generate the task breakdown, with task-driven 3D scene graph construction to generate a suitable representation of the environment. Our experiments show that ASHiTA performs significantly better than LLM baselines in breaking down high-level tasks into environment-dependent subtasks and is additionally able to achieve grounding performance comparable to state-of-the-art methods.

==> tex/hib_old.tex <==
%!TEX root = ../main.tex

\subsection{Hierarchical Information Bottleneck}
\label{appendix:hib_notes}

In general, the goal of robot perception is to take the sensor observations $\observations$
and compress them into a compact scene representation $\sgraph$ such that it suits the task $\tasks$ that the robot wants to perform.
Formally, it can be formulated as an information bottleneck~\cite{Tishby01accc-IB},
\begin{equation} \label{eq:scene_ib}
    \min I(\observations; \sgraph) - \beta I(\tasks; \sgraph)
\end{equation}

In some cases, it is possible to define the task with different resolutions,
by increasing or decreasing the specifications of the task.
Consequently, it should be also possible to find a scene representation that corresponds to \emph{each resolution of the task}.
We call each of these representations as a \emph{scene level}
and the collection of scene levels as a \emph{scene graph}.
Furthermore, a natural hierarchy forms if we assume that each scene level is a strict compression of its direct lower scene level.


\subsubsection{Derivation of Hierarchichal IB}
We can find a hierarchical scene representation
such that each layer of the hierarchy corresponds to 
different levels of abstractions of defined tasks.
To define this formally, we extend the information bottleneck as described in \eqref{eq:scene_ib} to
\begin{equation} 
\begin{split}
    \min &[I(\observations; \sgraph_1) + I(\sgraph_1; \sgraph_2) + \hdots + I(\sgraph_{n-1}; \sgraph_n) \\
    - &\beta (I(\tasks_1; \sgraph_1) + I(\tasks_2; \sgraph_2) + \hdots + I(\tasks_n; \sgraph_n)]
\end{split}   
\end{equation}
and we can define $\sgraph_0 = \observations$ so that we can write this more compactly:
\begin{equation}\label{eq:hib_app}
    \sum_{i=1}^n I(\sgraph_{i-1} ; \sgraph_i) - \beta \sum_{i=1}^n I(\tasks_i ; \sgraph_i)
\end{equation}

It might be tempting to simply apply the information bottleneck algorithm in succession in a bottom-up manner.
However, this fails to account for the "future" levels,
since the probability distribution of each level $\prob{\sgraph_i}$,
is dependent on the conditional probability $\prob{\sgraph_{i-1} | \sgraph_i}$.

The following is the derivation of the hierarchical information bottleneck,
referred to as \hib from here on.

Since each scene level is a strict compression of the previous level,
we have the Markov chain condition $\tasks_i \leftarrow \sgraph_0 \leftarrow \sgraph_1 \leftarrow \hdots \leftarrow \sgraph_n$ for all resolutions of the task description $\tasks_i$.

Writing down the conditional distributions, we have that,
\begin{equation}
    p(s_1) = \sum_{s_0\in \sgraph_0} p(s_1 | s_0) p(s_0)
\end{equation}
\begin{equation}
    p(s_1|t_1) = \sum_{s_0\in \sgraph_0} p(s_1 | s_0) p(s_0|t_1)
\end{equation}
\begin{equation}
    p(s_2) = \sum_{s_1 \in \sgraph_1}\sum_{s_0 \in \sgraph_0} p(s_2 | s_1)p(s_1 | s_0) p(s_0)
\end{equation}
\begin{equation}
    p(s_2|t_2) = \sum_{s_1\in \sgraph_1} \sum_{s_0 \in \sgraph_0} p(s_2 | s_1) p(s_1|s_0) p(s_0|t_2)
\end{equation}
Generalizing for level $n$ and some integer $k$ such that $ n > k > 0$,
\begin{equation}\label{eq:psn}
    p(s_n) = \sum_{s_k \in \sgraph_k}\sum_{s_{k-1} \in \sgraph_{k-1}} p(s_n | s_k) p(s_k | s_{k-1}) p(s_{k-1})
    % p(s_n) = \sum_{s_{n-1} \in \sgraph_{n-1}} p(s_n | s_{n-1}) p(s_{n-1})
    % p(s_n) = \sum_{s_{n-1} \in \sgraph_{n-1}} \hdots \sum_{s_1 \in \sgraph_1}\sum_{s_0 \in \sgraph_0} p(s_n | s_{n-1}) \hdots p(s_1 | s_0) p(s_0)
\end{equation}
\begin{equation}\label{psntn}
    p(s_n|t_n) = \sum_{s_k \in \sgraph_k} \sum_{s_{k-1} \in \sgraph_{k-1}} p(s_n | s_k) p(s_k|s_{k-1})p(s_{k-1}|s_0)p(s_0|t_n)
    % p(s_n|t_n) = \sum_{s_{n-1} \in \sgraph_{n-1}} \hdots \sum_{s_1 \in \sgraph_1}\sum_{s_0 \in \sgraph_0} p(s_n | s_{n-1}) \hdots p(s_1|s_0) p(s_0|t_n)
\end{equation}

Taking the derivative of the conditional distributions with respect to $p(s_1|o) \hdots p(s_k|s_{k-1})$,
\begin{equation}
    \frac{\delta p(s_1)}{\delta p(s_1 | s_0)} = p(s_0)
\end{equation}
\begin{equation}
    \frac{\delta p(s_1|t_1)}{\delta p(s_1 | s_0)} = p(s_0|t_1)
\end{equation}
\begin{equation}\label{eq:dpsn}
    \frac{\delta p(s_n)}{\delta p(s_k | s_{k-1})} = p(s_n | s_k)p(s_{k-1})
\end{equation}
\begin{equation}\label{eq:dpsntn}
    \frac{\delta p(s_n|t_n)}{\delta p(s_k | s_{k-1})} = p(s_n|s_k)p(s_{k-1}|s_0)p(s_0|t_n)
\end{equation}

The full Lagrangian expression for \eqref{eq:hib} (including Lagrange multipliers for the normalization of the conditional probabilities $p(s_i|s_{i-1})$ is,
\begin{equation}\label{eq:lagrangian}
\begin{split}
    \mathcal{L} &= \sum_{i=1}^n \{I(\sgraph_{i-1} ; \sgraph_i) - \beta I(\tasks_i ; \sgraph_i) \\
    &+ \sum_{s_{i-1}}\lambda (s_{i-1})[\sum_{s_i}p(s_i|s_{i-1}) - 1)]\}\\
\end{split}
\end{equation}

Recalling the definition for mutual information
\begin{equation}\label{eq:mutual_information}
\begin{split}
    I(X; Y) &= \sum_{x}\sum_{y}p(x, y) log(\frac{p(x, y)}{p(x) p(y)})\\
    &= \sum_{x}\sum_{y}p(x|y)p(y) log(\frac{p(x|y)}{p(x)})\\
\end{split}
\end{equation}

using logarithmic properties, we expand \eqref{eq:lagrangian} as,
\begin{equation}\label{eq:lagrangian_expanded}
\begin{split}
    \mathcal{L} &= \sum_{i=1}^n \{ \\
    &\sum_{s_{i-1}} p(s_{i-1}) \sum_{s_i} p(s_i | s_{i-1}) [log(p(s_i|s_{i-1})) - log(p(s_i))] \\
    &-\beta\sum_{t_i} p(t_i) \sum_{s_i} p(s_i | t_i) [log(p(s_i|t_i)) - log(p(s_i))] \\
    &+\sum_{s_{i-1}}\lambda (s_{i-1})[\sum_{s_i}p(s_i|s_{i-1}) - 1)]\} \\
\end{split}
\end{equation}

As a warm-up, let us first find the optimal clustering for the bottom level given by $p(s_1|s_0)$. 
Rewriting \eqref{eq:lagrangian_expanded},
\begin{equation}\label{eq:lagrangian_expanded_bottommost}
\begin{split}
    \mathcal{L} &= \sum_{s_0} p(s_0) \sum_{s_1} p(s_1 | s_0) [log(p(s_1|s_0)) - log(p(s_1))] \\
    +&\sum_{s_1} p(s_1) \sum_{s_2} p(s_2 | s_1) [log(p(s_2|s_1)) - log(p(s_2))] \\
    +&\sum_{i=3}^n \{ \\
    &\sum_{s_{i-1}} p(s_{i-1}) \sum_{s_i} p(s_i | s_{i-1}) [log(p(s_i|s_{i-1})) - log(p(s_i))] \} \\
    -&\beta\sum_{t_1} p(t_1) \sum_{s_1} p(s_1 | t_1) [log(p(s_1|t_1)) - log(p(s_1))] \\
    -&\beta\sum_{i=2}^n \{\sum_{t_i} p(t_i) \sum_{s_i} p(s_i | t_i) [log(p(s_i|t_i)) - log(p(s_i))] \} \\
    +&\sum_{i=1}^n \{\sum_{s_{i-1}}\lambda (s_{i-1})[\sum_{s_i}p(s_i|s_{i-1}) - 1)]\} \\
\end{split}
\end{equation}

Notice that the terms dependent on $p(s_1|s_0)$ are $p(s_1|s_0)$, $p(s_i)$ for $i > 0$, and $p(s_i|t_i)$.

From basic calculus, we can derive that
\begin{equation}
    \frac{df(x) log(f(x))}{dx} = \frac{df(x)}{dx}(log(f(x)) + 1)
\end{equation}

the derivative of the Lagrangian $\frac{\delta \mathcal{L}}{\delta p(s_1|s_0)}$ for fixed $s_1$ and $s_0$ is,

\begin{equation}
\begin{split}
    \frac{\delta \mathcal{L}}{\delta p(s_1|s_0)} &=
    p(s_0)[log(p(s_1|s_0)) + 1]
    - \frac{\delta p(s_1)}{\delta p(s_1|s_0)}[log(p(s_1)) + 1] \\
    +& \frac{\delta p(s_1)}{\delta p(s_1|s_0)}\sum_{s_2}p(s_2 | s_1) log(p(s_2|s_1)) \\
    &- \sum_{s_2} \frac{\delta p(s_2)}{\delta p(s_1|s_0)}[log(p(s_2)) + 1] \\
    +&\sum_{i=3}^n \{
    \sum_{s_{i-1}} \frac{\delta p(s_{i-1})}{\delta p(s_1|s_0)} \sum_{s_i} p(s_i | s_{i-1}) log(p(s_i|s_{i-1})) \\
    &- \sum_{s_i}\frac{\delta p(s_i)}{\delta p(s_1|s_0)}[log(p(s_i)) + 1] \} \\
    -&\beta\{ \sum_{t_1}p(t_1)\frac{\delta p(s_1|t_1)}{\delta p(s_1|s_0)}[log(p(s_1|t_1)) + 1] \\
    &-\frac{\delta p(s_1)}{\delta p(s_1|s_0)}[log(p(s_1)) + 1]) \}\\
    -&\beta\sum_{i=2}^n \{\sum_{t_i}p(t_i)\sum_{s_i}\frac{\delta p(s_i|t_i)}{\delta p(s_1|s_0)}[log(p(s_i|t_i)) + 1] \\
    &-\sum_{s_i}\frac{\delta p(s_i)}{\delta p(s_1|s_0)}[log(p(s_i)) + 1]) \} \\
    +&\lambda(s_0)
\end{split}
\end{equation}

Plugging in \eqref{eq:dpsn} and \eqref{eq:dpsntn},
\begin{equation}
\begin{split}
    \frac{\delta \mathcal{L}}{\delta p(s_1|s_0)} &=
    p(s_0)[log(p(s_1|s_0)) + 1]
    - p(s_0) [log(p(s_1)) + 1] \\
    +& p(s_0)\sum_{s_2}p(s_2 | s_1) log(p(s_2|s_1)) \\
    &- \sum_{s_2}p(s_2|s_1)p(s_0)[log(p(s_2)) + 1] \\
    +&\sum_{i=3}^n \{
    \sum_{s_{i-1}} p(s_{i-1}|s_1)p(s_0) \sum_{s_i} p(s_i | s_{i-1}) log(p(s_i|s_{i-1})) \\
    &- \sum_{s_i}p(s_i|s_1) p(s_0)[log(p(s_i)) + 1] \} \\
    -&\beta\{ \sum_{t_1}p(t_1)p(s_0|t_1)[log(p(s_1|t_1)) + 1] \\
    &-p(s_0)[log(p(s_1)) + 1]) \}\\
    -&\beta\sum_{i=2}^n \{\sum_{t_i}p(t_i)\sum_{s_i}p(s_i|s_1)p(s_0|t_i)[log(p(s_i|t_i)) + 1] \\
    &-\sum_{s_i}p(s_i|s_1)p(s_0)[log(p(s_i)) + 1]) \} + \lambda(s_0) \\
\end{split}
\end{equation}
simplifying and noting that $p(t_1)p(s_0|t_1) = p(s_0)p(t_1|s_0)$
\begin{equation}\label{eq:l_dir_simplified}
\begin{split}
    &\frac{\delta \mathcal{L}}{\delta p(s_1|s_0)}=\\
    & p(s_0) \{log(\frac{p(s_1|s_0)}{p(s_1)}) + \sum_{s_2}p(s_2 | s_1) log(\frac{p(s_2 | s_1)}{p(s_2)}) \\
    +& \sum_{i=3}^n \{ \sum_{s_{i-1}} p(s_{i-1}|s_1) \sum_{s_i} p(s_i | s_{i-1})log(\frac{p(s_i|s_{i-1})}{p(s_i)}) \} \\
    -& (n - 1) -\beta \sum_{t_1}p(t_1|s_0)log(\frac{p(s_1|t_1)}{p(s_1)}) \\
    -&\beta\sum_{i=2}^n \{\sum_{t_i}p(t_i|s_0)\sum_{s_i}p(s_i|s_1)log(\frac{p(s_i|t_i)}{p(s_i)}) \} + \lambda(s_0) \\
\end{split}
\end{equation}

With some rearranging, we can manipulate some of the task related terms as,
\begin{equation}\label{eq:kldiv_rewrite}
\begin{split}
    \sum_{t_i}&p(t_i|s_0)log(\frac{p(s_i|t_i)}{p(s_i)}) \\
    =&\sum_{t_i}p(t_i|s_0)log(\frac{p(t_i|s_i)}{p(t_i)})\\
    =&\sum_{t_i}p(t_i|s_0)[log(\frac{p(t_i|s_i)}{p(t_i|s_0)}) + log(\frac{p(t_i|s_0)}{p(t_i)})]\\
    =&-D_{KL}(p(t_i|s_i)||p(t_i|s_0)) + \sum_{t_i} p(t_i|s_0) log(\frac{p(t_i|s_0)}{p(t_i)})
\end{split}
\end{equation}

Notice that $p(s_i|s_1) log(\sum_{t_i} p(t_i|s_0) log(\frac{p(t_i|s_0)}{p(t_i)})$
is independent of $s_0$ and $s_1$.
Let us then define a new variable $\tilde{\lambda}$
\begin{equation}
\begin{split}
    &\tilde{\lambda} = \frac{\lambda(s_0)}{p(s_0)} - (n - 1) 
    - \beta \sum_{t_1}p(t_1|s_0) log(\frac{p(t_1|s_0)}{p(t_1)} \\
    -& \beta \sum_{i=2}^n \sum_{s_i} p(s_i | s_1) \sum_{t_i} p(t_i|s_0) log(\frac{p(t_i|s_0)}{p(t_i)})
\end{split}
\end{equation}
so that \eqref{eq:l_dir_simplified} becomes,
\begin{equation}\label{eq:l_dir_bottom_final}
\begin{split}
    &\frac{\delta \mathcal{L}}{\delta p(s_1|s_0)}=\\
    & p(s_0) \{log(\frac{p(s_1|s_0)}{p(s_1)}) + \sum_{s_2}p(s_2 | s_1) log(\frac{p(s_2 | s_1)}{p(s_2)}) \\
    +& \sum_{i=3}^n \{ \sum_{s_{i-1}} p(s_{i-1}|s_1) \sum_{s_i} p(s_i | s_{i-1})log(\frac{p(s_i|s_{i-1})}{p(s_i)}) \} \\
    +& \beta D_{KL}(p(t_1|s_1)||p(t_1|s_0)) \\
    +&\beta\sum_{i=2}^n \{\sum_{s_i}p(s_i|s_1)D_{KL}(p(t_i|s_i)||p(t_i|s_0)) \} + \tilde{\lambda} \} \\
\end{split}
\end{equation}

Setting $\frac{\delta \mathcal{L}}{\delta p(s_1|s_0)} = 0$,
we end up with
\begin{equation}\label{eq:hib_os1}
\begin{split}
    p(s_1&|s_0) = \frac{p(s_1)}{\mathcal{Z}} \exp[-\beta D_{KL}(p(t_1|s_1) || p(t_1|s_0)) \\
    &-\beta\sum_{i=2}^n\sum_{s_i}p(s_i|s_1)D_{KL}(p(t_i|s_i) || p(t_i|s_0)) \\
    &- \sum_{s_2}p(s_2 | s_1) log(\frac{p(s_2 | s_1)}{p(s_2)}) \\
    &- \sum_{i=3}^n \{ \sum_{s_{i-1}} p(s_{i-1}|s_1) \sum_{s_i} p(s_i | s_{i-1})log(\frac{p(s_i|s_{i-1})}{p(s_i)}) \}]
\end{split}
\end{equation}

As a sanity check, notice that if $n=1$, we are left with
\begin{equation}
    p(s_1|s_0) = \frac{p(s_1)}{\mathcal{Z}} \exp[-\beta D_{KL}(p(t_1|s_1) || p(t_1|s_0))]
\end{equation}
with $\tilde{\lambda}(s_0) = \frac{\lambda(s_0)}{p(s_0)} - \beta\sum_{t_1}p(t_1|s_0) log(\frac{p(t_1|s_0)}{p(t_1)})$,
which is the well known solution for IB\cite{Tishby01accc-IB}.

In the case where $ n > 1$,
the result here indicates that the KL-divergence of the i-th layer is still accounted for
even when solving for the bottom layer,
and are weighted somewhat intuitively according to $p(s_i|s_1)$.
Moreover, $p(s_1|s_0)$ also encourages the "spreading out" of the cluster assignments
(\ie third and fourth term decreases the magnitude of the negative exponent in \eqref{eq:hib_os1} if they approach $0$, thereby increasing $p(s_1|s_0)$.

To derive $p(s_k|s_{k-1})$ for some arbitrary level $k$,
we rewrite \eqref{eq:lagrangian_expanded} as
\begin{equation}\label{eq:lagrangian_expanded_k}
\begin{split}
    \mathcal{L} &= \sum_{i=1}^{k-1} \{ \\
    &\sum_{s_{i-1}} p(s_{i-1}) \sum_{s_i} p(s_i | s_{i-1}) [log(p(s_i|s_{i-1})) - log(p(s_i))] \} \\
    +&\sum_{s_{k-1}} p(s_{k-1}) \sum_{s_k} p(s_k | s_{k-1}) [log(p(s_k|s_{k-1})) - log(p(s_k))] \\
    +&\sum_{s_{k}} p(s_{k}) \sum_{s_{k+1}} p(s_{k+1} | s_{k}) [log(p(s_{k+1}|s_{k})) - log(p(s_{k+1}))] \\
    +&\sum_{i=k+2}^n \{ \\
    &\sum_{s_{i-1}} p(s_{i-1}) \sum_{s_i} p(s_i | s_{i-1}) [log(p(s_i|s_{i-1})) - log(p(s_i))] \} \\
    -&\beta\sum_{i=1}^{k-1} \{\sum_{t_i} p(t_i) \sum_{s_i} p(s_i | t_i) [log(p(s_i|t_i)) - log(p(s_i))] \} \\
    -&\beta\sum_{t_k} p(t_k) \sum_{s_k} p(s_k | t_k) [log(p(s_k|t_k)) - log(p(s_k))] \\
    -&\beta\sum_{i=k + 1}^n \{\sum_{t_i} p(t_i) \sum_{s_i} p(s_i | t_i) [log(p(s_i|t_i)) - log(p(s_i))] \} \\
    +&\sum_{i=1}^{k-1} \{\sum_{s_{i-1}}\lambda (s_{i-1})[\sum_{s_i}p(s_i|s_{i-1}) - 1)]\} \\
    +&\sum_{s_{k-1}}\lambda (s_{k-1})[\sum_{s_k}p(s_k|s_{k-1}) - 1)]\} \\
    +&\sum_{i=k+1}^n \{\sum_{s_{i-1}}\lambda (s_{i-1})[\sum_{s_i}p(s_i|s_{i-1}) - 1)]\} \\
\end{split}
\end{equation}
the derivative of the Lagrangian $\frac{\delta \mathcal{L}}{\delta p(s_k|s_{k-1})}$ for fixed $s_k$ and $s_{k-1}$ is,
\begin{equation}
\begin{split}
    &\frac{\delta \mathcal{L}}{\delta p(s_k|s_{k-1})}\\
    =&p(s_{k-1})[log(p(s_k|s_{k-1})) + 1] \\
    &- \frac{\delta p(s_k)}{\delta p(s_k|s_{k-1})}[log(p(s_k)) + 1] \\
    +& \frac{\delta p(s_k)}{\delta p(s_k|s_{k-1})}\sum_{s_{k+1}}p(s_{k+1} | s_k) log(p(s_{k+1}|s_k)) \\
    &- \sum_{s_{k+1}} \frac{\delta p(s_{k+1})}{\delta p(s_k|s_{k-1})}[log(p(s_{k+1})) + 1] \\
    +&\sum_{i=k+2}^n \{
    \sum_{s_{i-1}} \frac{\delta p(s_{i-1})}{\delta p(s_k|s_{k-1})} \sum_{s_i} p(s_i | s_{i-1}) log(p(s_i|s_{i-1})) \\
    &- \sum_{s_i}\frac{\delta p(s_i)}{\delta p(s_k|s_{k-1})}[log(p(s_i)) + 1] \} \\
    -&\beta\{ \sum_{t_k}p(t_k)\frac{\delta p(s_k|t_k)}{\delta p(s_k|s_{k-1})}[log(p(s_k|t_k)) + 1] \\
    &-\frac{\delta p(s_k)}{\delta p(s_k|s_{k-1})}[log(p(s_k)) + 1]) \}\\
    -&\beta\sum_{i=k+1}^n \{\sum_{t_i}p(t_i)\sum_{s_i}\frac{\delta p(s_i|t_i)}{\delta p(s_k|s_{k-1})}[log(p(s_i|t_i)) + 1] \\
    &-\sum_{s_i}\frac{\delta p(s_i)}{\delta p(s_k|s_{k-1})}[log(p(s_i)) + 1]) \} +\lambda(o)
\end{split}
\end{equation}

Plugging in \eqref{eq:dpsn} and \eqref{eq:dpsntn},
\begin{equation}\label{eq:k_level_halfway}
\begin{split}
    &\frac{\delta \mathcal{L}}{\delta p(s_k|s_{k-1})}\\
    =&p(s_{k-1}) \{ log(\frac{p(s_k|s_{k-1})}{p(s_k)}) \\
    +& \sum_{s_{k+1}}p(s_{k+1}|s_k) log(\frac{p(s_{k+1}|s_k)}{p(s_{k+1})}) \\
    +&\sum_{i=k+2}^n \{
    \sum_{s_{i-1}} p(s_{i-1}|s_k)\sum_{s_i} p(s_i | s_{i-1}) log(\frac{p(s_i|s_{i-1})}{p(s_i)}) \}\\
    &- (n-1) \\
    % TODO CHECK THIS
    -&\beta\{\sum_{t_k}p(t_k)p(s_{k-1}|o)p(o|t_k)[log(p(s_k|t_k)) + 1] \\
    &-p(s_{k-1})[log(p(s_k)) + 1]) \}\\
    -&\beta\sum_{i=k+1}^n \{\\
    &\sum_{t_i}p(t_i)\sum_{s_i}p(s_i|s_k)p(s_{k-1}|s_0)p(s_0|t_i)[log(p(s_i|t_i)) + 1] \\
    &-\sum_{s_i}p(s_i|s_k)p(s_{k-1})[log(p(s_i)) + 1]) \} +\lambda(s_0)
\end{split}
\end{equation}

We can rewrite $p(t_k)p(s_{k-1}|o)p(o|t_k)$ as
\begin{equation}
    p(t_k)p(s_{k-1}|t_k)= p(s_{k-1})p(t_k|s_{k-1})
\end{equation}
which allows us to simplify \eqref{eq:k_level_halfway} further as,
\begin{equation}\label{eq:k_level_deriv}
\begin{split}
    &\frac{\delta \mathcal{L}}{\delta p(s_k|s_{k-1})}\\
    =&p(s_{k-1}) \{ log(\frac{p(s_k|s_{k-1})}{p(s_k)}) \\
    +& \sum_{s_{k+1}}p(s_{k+1}|s_k) log(\frac{p(s_{k+1}|s_k)}{p(s_{k+1})}) \\
    +&\sum_{i=k+2}^n \{
    \sum_{s_{i-1}} p(s_{i-1}|s_k)\sum_{s_i} p(s_i | s_{i-1}) log(\frac{p(s_i|s_{i-1})}{p(s_i)}) \\
    &- (n-1) \\
    -&\beta\sum_{t_k}p(t_k|s_{k-1})log(\frac{p(s_k|t_k)}{p(s_k)}) \\
    -&\beta\sum_{i=k+1}^n \{
    \sum_{t_i}\sum_{s_i}p(s_i|s_k)p(t_i|s_{k-1})log(\frac{p(s_i|t_i)}{p(s_i)}) \} \} + \lambda(o)
\end{split}
\end{equation}

Again we can perform some symbolic manipulation,
\begin{equation}
\begin{split}
    &p(t_i|s_{k-1})log(\frac{p(s_i|t_i)}{p(s_i)}) = -D_{KL}(p(t_i|s_{k-1}) || p(t_i|s_i)) \\
    &+ \sum_{t_i}p(t_i|s_{k-1})log(\frac{p(t_i|s_{k-1}}{p(t_i)})) \\
\end{split}
\end{equation}

Hence we have that 
\begin{equation}
\begin{split}
    p(s_k&|s_{k-1}) = \frac{p(s_k)}{\mathcal{Z}} \exp[-\beta D_{KL}(p(t_k|s_k) || p(t_k|s_{k-1})) \\
    &-\beta\sum_{i=k+1}^n\sum_{s_i}p(s_i|s_k)D_{KL}(p(t_i|s_i) || p(t_i|s_{k-1})) \\
    &- \sum_{s_{k+1}}p(s_{k+1} | s_k) log(\frac{p(s_{k+1} | s_k)}{p(s_{k+1})}) \\
    &- \sum_{i=k+2}^n \{ \sum_{s_{i-1}} p(s_{i-1}|s_k) \sum_{s_i} p(s_i | s_{i-1})log(\frac{p(s_i|s_{i-1})}{p(s_i)}) \}]
\end{split}
\end{equation}

and note that the last two terms are not directly dependent on $s_k$ and $s_{k-1}$ so we can incorporate that into the normalization factor: 
\begin{equation}\label{eq:hib_sk}
\begin{split}
    p(s_k&|s_{k-1}) = \frac{p(s_k)}{\mathcal{Z}} \exp[-\beta D_{KL}(p(t_k|s_k) || p(t_k|s_{k-1})) \\
    &-\beta\sum_{i=k+1}^n\sum_{s_i}p(s_i|s_k)D_{KL}(p(t_i|s_i) || p(t_i|s_{k-1})) ] \\
\end{split}
\end{equation}

and easy to check that for $k = 1$, \eqref{eq:hib_sk} is equivalent to \eqref{eq:hib_os1}.

Now we can write down our set of self-consistent equations for step $k$ for iteration $i$:
\begin{equation}\label{eq:hib_cases}
    \begin{cases}
        & p_i(s_k|s_{k-1}) = \frac{1}{\mathcal{Z}} p(s_k) \exp(\beta d) \\
        & p_{i+1}(s_k) = \sum_{s_{k-1}}p(s_{k-1})p(s_k | s_{k-1}) \\
        & p_{i+1}(t_k|s_k) = \sum_{s_{k-1}}p(t_k|s_{k-1})p(s_{k-1}|s_k)
    \end{cases}
\end{equation}

In practice, we apply \eqref{eq:hib_cases} in a bottom-up fashion for each iteration.

\myParagraph{Convergence}
Here, we give a sketch of the proof for convergence. From the definition of mutual information,
\begin{equation}
I(X; Y) = - \sum_{x\in X} \sum_{y \in Y} p(x, y) \log \left( \frac{p(x)p(y)}{p(x, y} \right),
\end{equation}
As 
\begin{equation}
\sum_{x\in X} \sum_{y \in Y} p(x, y) = 1
\end{equation}
and the fact the negative logarithm $f(x) = -\log (x)$ is convex with $f'' (x) \geq 0$ for all $x>0$, we can apply Jensen's Inequality to show
\begin{align}
I(X; Y) &\geq& -\log \left( \sum_{x\in X} \sum_{y \in Y} p(x, y) \frac{p(x)p(y)}{p(x, y)}  \right) \\
&=& - \log \left( \sum_{x\in X} \sum_{y \in Y} p(x) p(y)  \right) = 0
\end{align}

As mutual information is always non-negative, the functional \eqref{eq:hib}, as a sum of non-negative terms, is bounded from below, preventing it from decreasing indefinitely. 

Each iteration step is independent and minimizes the functional with respect to one of the distributions $p(s_k|s_{k-1})$, $p(s_k)$, and $p(t_k|s_k)$ while keeping the others fixed, such that $\mathcal{L}_{t+1} \leq \mathcal{L}_t$. Since $L_t$ is non-increasing and bounded below, the sequence converges to a limit $\mathcal{L}^*$:
\begin{equation}
    \lim_{t \rightarrow \infty} \mathcal{L}_t = \mathcal{L}^*
\end{equation}
For fixed $p(t_k|s_k)$, $\mathcal{L}$ is convex in $p(s_k|s_{k-1})$; for fixed $p(s_k|s_{k-1})$, $\mathcal{L}$ is convex in $p(t_k|s_k)$. Given that $\mathcal{L}_t$ converges by decreases monotonically and is bounded below, with each update step minimizing $\mathcal{L}$ due to convexity, we expect $\mathcal{L}$ to converge to a (local) minimum. As $\mathcal{L}$ is not jointly convex in all distributions simultaneously, we also expect that the algorithm may converge to different local minima depending on initialization, and convergence does not imply the uniqueness of the solution as multiple local optima may exist.

\subsubsection{Example Compared to Applying IB sequentially}
Given uniformly distributed discrete random variables $X$, $Y_1$, and $Y_2$
with sample space $\{ 1, \hdots , 8 \}$, $\{ 1, \hdots , 4 \}$, and $\{ 1, 2 \}$ respectively.
Let's say we want to find two different abstractions of $X$: $Z_1$, and $Z_2$ with respect to $Y_1$ and $Y_2$.

Starting with an easy case, we define the conditional probabilities
\begin{equation}
    p(y_1 = i|x) =
    \begin{cases}
        1, & \text{if } 2(i-1) < x \leq 2i, \\
        0, &\text{otherwise}
    \end{cases}
\end{equation}
\begin{equation}
    p(y_2 = i|x) =
    \begin{cases}
        1, & \text{if } 4(i-1) < x \leq 4i, \\
        0, &\text{otherwise}
    \end{cases}
\end{equation}

It is easy to see that both applying generic IB sequentially or applying HIB
will give us $\prob{Z_1|X}$ and $\prob{Z_2|Z_1}$ that form 4 clusters for the first level,
and 2 clusters for the second level (assuming $\beta$ = 1).

Let us perturb $\prob{Y_1|X}$ a little for $x \in \{ 4, 5 \}$, such that
$p(y_1 = 2 |x) = 0.5$ and $p(y_1 = 3 |x) = 0.5$ for $x = 4$ and $x = 5$.
In this case, generic IB will form three clusters from $\prob{Z_1|X}$,
but HIB will still maintain four clusters due to the influence from $\prob{Y_2|X}$.

\subsubsection{\hdib}
Following the arguments in~\cite{Strouse15neuralComputation-DIB}, we can similarly define a "generalized" \hib problem,
rewriting \eqref{eq:hib} as
\begin{equation}
    \sum_{i=1}^n [H(\sgraph_i) - \alpha H(\sgraph_i | \sgraph_{i-1})] - \beta \sum_{i=1}^n I(\tasks_i ; \sgraph_i)
\end{equation}

Expanding and then following a similar derivation as \hib, we eventually obtain 
\begin{equation}\label{eq:hdib_sk}
\begin{split}
    p_{\alpha}(s_k&|s_{k-1}) = \frac{1}{\mathcal{Z}} \exp[\frac{1}{\alpha}log(p(s_k)) -\beta D_{KL}(p(t_k|s_k) || p(t_k|s_{k-1})) \\
    &-\beta\sum_{i=k+1}^n\sum_{s_i}p(s_i|s_k)D_{KL}(p(t_i|s_i) || p(t_i|s_{k-1})) ] \\
\end{split}
\end{equation}

If $\alpha = 1$, it is obvious that we recover the previously derived equation for \hib.
If $\alpha \rightarrow 0$, the argument of the exponential blows up, hence,
\begin{equation}
\begin{split}
    \lim_{\alpha \rightarrow 0}& p_{\alpha}(s_k|s_{k-1}) = f(s_{k-1})\\
    =& \argmax_{s_k} (log(p(s_k)) -\beta D_{KL}(p(t_k|s_k) || p(t_k|s_{k-1})) \\
    &-\beta\sum_{i=k+1}^n\sum_{s_i}p(s_i|s_k)D_{KL}(p(t_i|s_i) || p(t_i|s_{k-1})))
\end{split}
\end{equation}

We can write down our set of self-consistent equations for step $k$ for iteration $i$ for \hdib:
\begin{equation}\label{eq:hdib_cases}
    \begin{cases}
        & p_i(s_k|s_{k-1}) = \delta(s_k - f(s_{k-1}))\\
        & p_{i+1}(s_k) = \sum_{s_{k-1}}p(s_{k-1})p(s_k | s_{k-1}) \\
        & p_{i+1}(t_k|s_k) = \sum_{s_{k-1}}p(t_k|s_{k-1})p(s_{k-1}|s_k)
    \end{cases}
\end{equation}


% In other words, let's consider two scene graph representations, $\sgraph$ and $\sgraph^+$,
% which corresponds to two set of task distributions $\tasks$ and $\tasks^+$.
% Let us assume that $\sgraph \subseteq \sgraph^+$ and $\tasks \subseteq \tasks^+$.
% We can write down a set of information bottleneck equations:
% \begin{equation}
% \begin{split}
%     &\min I(\map ; \sgraph^+) - \beta I(\tasks^+ ; \sgraph^+) \\
%     &\min I(\sgraph^+; \sgraph) - \beta I (\tasks ; \sgraph) \\
% \end{split}
% \end{equation}

% Intuitively, as we ascend the hierarchy,
% the scene graph $\sgraph^+$ is compressed into a scene graph $\sgraph$ that corresponds to a condensed version
% of the tasks.

% The self-consistent equations then becomes
% \begin{equation}
% \begin{split}
%     &p(t^+ | s^+) = \frac{1}{p(s^+)} \sum_{s^+ \in \sgraph^+} p(t^+ | m) p(s^+ | m) p(m)\\
%     &p(s^+ | m) = \frac{p(s^+)}{Z(m, \beta)} \exp [-\beta \sum_{t^+ \in \tasks^+} p(t^+ | m) \log \frac{p(t^+|m)}{p(t^+|s^+}] \\
%     &p(t | s^+) = \frac{1}{p(s^+)}\sum_{s^+}p(t|m)p(s^+|m)p(m) \\
%     &p(t | s) = \frac{1}{p(s)} \sum_{s \in \sgraph} p(t | s^+) p(s | s^+) p(s^+) \\
%     &p(s | s^+) = \frac{p(s)}{Z(s^+, \beta)} \exp [-\beta \sum_{t \in \tasks} p(t | s^+) \log \frac{p(t|s^+)}{p(t|s)}] \\
%     &p(s | m) = \frac{1}{p(s^+} \sum_{s^+} p(s|s^+) p(s^+|m) p(m) \\
% \end{split}
% \end{equation}

% We also note that for each level of the hierarchy to be optimal, we can enforce that
% \begin{equation}
% \begin{split}
%     p(t | s) &= \frac{1}{p(s)} \sum_{s^+} p(t | s^+) p(s | s^+) p(s^+) \\
%     &= \frac{1}{p(s)} \sum_{m} p(t | m) p(s | m) p(m)
% \end{split}
% \end{equation}
% \yc{Polish this to get a bottom-up, top-down refinement algorithm.}

% \subsection{Formalizing Task-Driven Scene Graphs via Inference}
% \yc{archived for now.}

% Let us define $\MS$ as a scene graph, $\MT = \{T_k\}$ as a list of user-defined tasks,
% $\bf{m}$ as the dense or sparse map of the environment, and $\M\Omega$ as a (vision) foundation model.
% A task-driven scene graph can be formally defined as,
% \begin{equation}\label{eq:task_driven_map}
%     \hat{\MS}_{\text{MAP}}(\MT, \bf{m}, \M\Omega) = \argmax_{\MS} \prob{\MS|\MT, \bf{m}, \M\Omega}
% \end{equation}

% Using Bayes' rule, we can manipulate \eqref{eq:task_driven_map} further
% \begin{equation}
% \begin{split}
%     \hat{\MS}_{\text{MAP}} &= \argmax_{\MS} \prob{\MS|\MT, \bf{m}, \M\Omega} \\
%     &= \argmax_{\MS} \prob{\MT|\MS, \bf{m}, \M\Omega} \prob{\MS, \bf{m}, \M\Omega} \\
%     &= \argmax_{\MS} \prob{\MT|\MS, \bf{m}, \M\Omega} \prob{\MS|\bf{m}}\prob{\bf{m}}\prob{\M\Omega} \\
% \end{split}
% \end{equation}

% The probability of $\M\Omega$ is difficult to characterize, so for now we assume that the information of the model
% is directly encoded in the tasks, the map, and the scene graph; hence,
% \begin{equation}
%     \hat{\MS}_{\text{MAP}} = \argmax_{\MS} \prob{\MT|\MS, \bf{m}} \prob{\MS|\bf{m}}\prob{\bf{m}} \\
% \end{equation}

% We make the generalizable assumption that the scene graph
% is composed of nodes $S_i$ such that $\MS = \{S_i\}$
% and the map is composed of independent entities (landmarks, points, or faces) such that $\bf{m} = \{m_i\}$.
% Assuming that the user-defined tasks are independent,
% \begin{equation}
%     \prob{\MT|\MS, \bf{m}} = \prod_{k}\prob{T_k| \MS, \bf{m}}
% \end{equation}

% We rewrite \eqref{eq:task_driven_map} as,
% \begin{equation}\label{eq:task_driven_expanded}
% \begin{split}
%     &\hat{\MS}_{\text{MAP}} = \\
%     &\argmax_{\MS} 
%     (\prod_{k}\prob{T_k| \MS, \bf{m}}) \prob{\MS|\bf{m}} \prod_j\prob{m_j}
% \end{split}
% \end{equation}

% Let us define $\MS$ as a scene graph, $\MT = \{T_k\}$ as a list of user-defined tasks,
% $\bf{m}$ as the dense or sparse map of the environment, and $\M\Omega$ as a (vision) foundation model.
% A task-driven scene graph can be formally defined as,
% \begin{equation}\label{eq:task_driven_map}
%     \hat{\MS}_{\text{MLE}}(\MT, \bf{m}, \M\Omega) = \argmax_{\MS} \prob{\MT|\MS, \bf{m}, \M\Omega}
% \end{equation}

% \yc{MLE can be solved via EM and Slonim showed that under certain conditions it is equivalent to IB.}

% \subsection{Formalizing Task-Driven Scene Graphs via IB}

% Given the world $\world$ and observations $\observations$.
% We can obtain some intermediate dense or sparse map representation $\map$
% and a scene graph representation $\sgraph$.
% We can also define the set of tasks as $\tasks$.
% We can sketch the information theoretic measures of the setup as shown in Fig.~\ref{fig:distribution}.

% \begin{figure}[t]
% \centering
% \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figures/distribution_sketch.pdf}
% \caption{Sketch of the information theoretic measures of the world $\world$, the robot observations $\observations$, the tasks $\tasks$, some map representation $\map$, and the scene graph $\sgraph$.}
% \label{fig:distribution}
% \end{figure}

% In general, robot perception seeks to compress the information of the world such that it is compact enough to fit on a mobile robot, but also contains sufficient information to carry out required tasks.
% Simply put, we can write this as the Information Bottleneck problem,
% \begin{equation} \label{eq:world_ib}
%     \min I(\world; \sgraph) - \beta I(\tasks; \sgraph)
% \end{equation}
% which intuitively can be seen precisely as the optimization to compress the scene representation while preserving
% the task relevance.
% It can also be seen as the minimization of part of the circle (that represent the entropy $H(S)$) that does not overlap with the yellow circle: in other words, minimizing $H(\sgraph | \tasks)$,
% the conditional entropy  of the scene graph given the tasks.

% However, the information of $\mathcal{W}$ or even $\mathcal{O}$ is difficult to characterize.
% Let us instead write this in terms of intermediate map representation $\map$.

% \begin{equation}\label{eq:ib_rewrite}
% \begin{split}
%     \min [& I(\world; \sgraph) - \beta I(\tasks; \sgraph) ]\\
%     &= \min [ H(\sgraph) - \beta (I(\map ; \sgraph; \tasks) + I(\sgraph ; \tasks | \map)) ] \\
%     &= \min [ H(\sgraph) - \beta (I(\map ; \sgraph) - I(\map ; \sgraph | \tasks) + I(\sgraph ; \tasks | \map))]\\
%     &= \min [ H(\sgraph) - \beta (I(\map ; \tasks) - I(\map ; \tasks | \sgraph) + I(\sgraph ; \tasks | \map))]\\
% \end{split}
% \end{equation}

% Expanding $I(\map; \tasks | \sgraph)$ and $H(\sgraph)$
% \begin{equation}
% \begin{split}
%     I(\map; \tasks | \sgraph) = &I(\map; \tasks) + H(\sgraph | \map) \\
%     &+ H(\sgraph | \tasks) - H(\sgraph | \map, \tasks) - H(\sgraph) \\
%     = &I(\map; \tasks) -I(\sgraph; \tasks) + I(\sgraph ; \tasks | \map)
% \end{split}
% \end{equation}
% \begin{equation}\label{eq:sgraph_entropy}
% \begin{split}
%     H(\sgraph) &= I(\map; \sgraph) - H(\map) + H(\map; \sgraph)\\
%     &= I(\map; \sgraph) - H(\map) + H(\sgraph | \map) + H(\map)\\
%     &= I(\map; \sgraph) + H(\sgraph | \map)
% \end{split}
% \end{equation}

% We can finally rewrite \eqref{eq:ib_rewrite} as,
% \begin{equation}\label{eq:general_ib}
% \begin{split}
%       \min [& I(\world; \sgraph) - \beta I(\tasks; \sgraph) ]\\
%     &= \min [ I(\map ; \sgraph) + H(\sgraph | \map) - \beta (I(\sgraph; \tasks)) ] \\  
% \end{split}
% \end{equation}

% In CLIO, we assumed that the scene graph is a strict compression of the intermediate map representation ($H(\sgraph | \map) = 0$); hence \eqref{eq:general_ib} becomes
% \begin{equation}
%     \min I(\map; \sgraph) - \beta I(\tasks; \sgraph)
% \end{equation}
% which is another IB formulation that uses the intermediate map as the uncompressed signal.

% \eqref{eq:general_ib} accounts for the case where the intermediate map does not contain all the information.
% In our case, this terms allows us to account for clustering as more than a simple compression.

% \yc{This should maybe overcome the problem with CLIP segments. But need to figure out how to model without requerying at different hierarchies. }

% \yc{We show that self-consistent equations can be derived to solve \eqref{eq:general_ib}.}


%%% Archived

% \subsection{CLIO and Information Bottleneck}
% In Clio, we made the assumption that scene graph nodes are independent,
% \begin{equation}
%     \prob{\MS|\bf{m}} = \prod_i \prob{S_i | \bf{m}} = \prod_i \sum_j \prob{S_i | m_j}
% \end{equation}
% and also that the scene graph is strictly losing task relevance compared to the map entities,
% \begin{equation}
%     \prob{\MT|\MS, \bf{m}} = \prob{\MT|\bf{m}} = \prod_k \sum_j \prob{T_k | m_j}
% \end{equation}

% With these assumptions, \eqref{eq:task_driven_expanded}
% becomes,
% \begin{equation}
% \begin{split}
%     &\hat{\MS}_{\text{MAP}} = \\
%     &\argmax_{\MS} 
%     (\prod_{k}\sum_{j}\prob{T_k|m_j}) \prod_i \sum_j \prob{S_i | m_j} \prod_j\prob{m_j}
% \end{split}
% \end{equation}

% To find $\MS$, CLIO solves the Information Bottleneck 
% for $\prob{\MS | \bf{m}}$.
% The Information Bottleneck can be written with our definitions as,
% \begin{equation}
%     \argmin_{\prob{S_i|m_j}} I(m; S) - \beta I(S; T)
% \end{equation}

% Expanding, we get,
% \begin{equation}
% \begin{split}
%     \argmin_{\prob{S_i|m_j}} &\sum_j \sum_i \prob{m_j}\prob{S_i | m_j} \log(\frac{\prob{S_i|m_j}}{\prob{S_i}}) \\
%     - &\beta \sum_i \sum_k \prob{S_i}\prob{T_k|S_i}\log (\frac{\prob{T_k|Si}}{\prob{T_k}})
% \end{split}
% \end{equation}

% Manipulating this expression, we show that we can get \yc{TODO. Slonim 02 used EM to demonstrate some equivalence between MLE and IB when applying the EM alg}.

% Moreover, CLIO uses the Agglomerative Information Bottleneck method,
% which is a hard clustering method that assumes $\beta \to \infty$ and introduce another heuristic stopping condition.



==> tex/objects_regions.tex <==
%!TEX root = ../main.tex
\begin{table}[h]{%
    \begin{tabular}{cl cc cccc}
    \toprule
    &  & \multicolumn{2}{c}{Objects} & \multicolumn{4}{c}{Regions.} \\
    \cmidrule(r){3-4} \cmidrule(r){5-8}
    Scene & Method & R & P & R & P & Sem R & Sem P \\
    \midrule
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{824}}} 
    & Hydra & - & - & - & - & - & - \\
    & HOV-SG & - & - & - & - & - & - \\
    & ASHiTA & 17.0 & 65.0 & 9.0 & 21.0 & 8.0 & 23.0 \\
    \midrule 
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{829}}} 
    & Hydra & - & - & - & - & - & - \\
    & HOV-SG & - & - & - & - & - & - \\
    & ASHiTA & 15.0 & 48.0 & 9.0 & 16.0 & 10.0 & 20.0 \\
    \midrule 
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{843}}} 
    & Hydra & - & - & - & - & - & - \\
    & HOV-SG & - & - & - & - & - & - \\
    & ASHiTA & 10.0 & 37.0 & 5.0 & 13.0 & 4.0 & 21.0 \\
    \midrule 
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{847}}} 
    & Hydra & - & - & - & - & - & - \\
    & HOV-SG & - & - & - & - & - & - \\
    & ASHiTA & 12.0 & 60.0 & 7.0 & 21.0 & 5.0 & 37.0 \\
    \midrule 
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{849}}} 
    & Hydra & - & - & - & - & - & - \\
    & HOV-SG & - & - & - & - & - & - \\
    & ASHiTA & 9.0 & 50.0 & 3.0 & 17.0 & 3.0 & 31.0 \\
    \midrule 
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{861}}} 
    & Hydra & - & - & - & - & - & - \\
    & HOV-SG & - & - & - & - & - & - \\
    & ASHiTA & 11.0 & 49.0 & 3.0 & 13.0 & 3.0 & 16.0 \\
    \midrule 
    \end{tabular}}
    \caption{Objects and Regions compared to existing task-agnostic scene graph pipelines.}
\end{table}

==> tex/task_eval_full_scene.tex <==
%!TEX root = ../main.tex
\begin{table}%
    \setlength{\tabcolsep}{2pt}
    \centering
    \begin{tabular}{c ccc}
    \toprule
    Method & s-rec (\%) & s-prec (\%) & t-acc (\%) \\
    \midrule
    \midrule
    Hydra + GPT & 2.7 & 3.16 & 1.95 \\
    HOV-SG + GPT & 0.23 & 0.47 & 0.0 \\
    ASHiTA & - & - & - \\
    \rowcolor{gray!20}
    ASHiTA (GT Pos) & 1.63 & 3.51 & 1.46 \\
    \rowcolor{blue!10}
    Hydra (GT Seg)~\cite{Hughes22rss-hydra} + GPT & 3.58 & 3.71 & \bf{5.37} \\
    \rowcolor{blue!10}
    ASHiTA (GT Pos + Txt Emb) & \bf{6.32} & \bf{7.76} & 4.88 \\
\midrule 
    \midrule 
    \end{tabular}
    \caption{\yc{This might not be worth keeping?} Evaluation of Hierarchical Task Analysis without knowing the region.\label{tab:full_task_eval}}
\end{table}
